Diffusion Structures for Architectural Stripe Pattern Generation

We present Diffusion Structures, a family of resilient shell structures from the eigenfunctions of a pair of novel diffusion operators. This approach is based on Michell's theorem but avoids expensive non-linear optimization with computation that amounts to constructing and solving two generalized eigenvalue problems to generate two sets of stripe patterns. This structure family can be generated quickly, and navigated in real-time using a small number of tuneable parameters.

==> sections/background.tex <==
\section{Background}

Before describing our method, we begin with some background on Michell trusses, diffusion operators in geometry processing, and the connection between the two.

\subsection{Michell Trusses}

An early method for structural optimization originated from \citet{michell1904}, who discovered that structures with optimal strength-to-weight ratios have material which follows the principal directions of the Cauchy stress tensors induced by loading conditions.
Such structures are known as \emph{Michell trusses}.

Despite this method being over a century old, computing Michell trusses is not straightforward, since analytical solutions do not exist in general.
The description above invokes a picture of integrating over vector fields, but extracting the vector fields is challenging due to tensor singularities in isotropic regions, where the principal directions are not unique.
However, this does not imply that an arbitrary set of orthogonal directions can be used at isotropic points: a non-smooth vector field produces visible artifacts in the resulting integration.
While these vector fields can be smoothed, ensuring fidelity with the anisotropic data requires an expensive nonlinear optimization.
To avoid these difficulties, we seek a holistic approach that works with tensor data directly and thus implicitly handles tensor singularities.
For this, we turn to \emph{diffusion operators}.

\subsection{Discrete Diffusion Operators}

The (continuous) diffusion equation is $\frac{\partial u}{\partial t} = D \Delta u$, where $D$ is a positive semi-definite tensor field.
Unlike the typical Laplace operator $\Delta$, this anisotropic Laplace operator $D \Delta$ encodes transmission propensity at each point as a local metric (\am{I don't know how exactly this imposed metric interacts with the metric of the domain}).
In computer graphics, discrete anisotropic Laplacians have been used for shape analysis~\cite{andreux2014}, which take per-face symmetric tensor fields as input along with the surface geometry.
To ensure the resulting matrix is negative semi-definite, the tensor field must be \emph{remapped} to be positive semi-definite everywhere.
The simplest way of doing this is flipping all negative eigenvalues to be positive, but we use a somewhat more involved procedure (see~\ref{sec:rescale}).

The connection between Michell trusses and diffusion is to view structural design as a physical process, where material diffuses based on the stress tensors.
In this way, material flows along the principal directions to form the trusses.

